Distributed Graph Automata

Inspired by distributed algorithms, we introduce a new class of finite graph automata that recognize precisely the graph languages definable in monadic second-order logic. For the cases of words and trees, it has been long known that the regular languages are precisely those definable in monadic second-order logic. In this regard, the automata proposed in the present work can be seen, to some extent, as a generalization of finite automata to graphs. Furthermore, we show that, unlike for finite automata on words and trees, the deterministic, nondeterministic and alternating variants of our automata form a strict hierarchy with respect to their expressive power. For the weaker variants, the emptiness problem is decidable.

==> fig/graph_templates.tex <==
%%% TeX-master: "../masterarbeit"

\newcommand{\pentagraphPic}[8]{
  \begin{tikzpicture}[lgraph,#1]
    \node[lnode] (u) {#3};
    \node[lnode] (v) at ([shift={(90:#2)}]u) {#4};
    \node[lnode] (w) at ([shift={(18:#2)}]u) {#5};
    \node[lnode] (x) at ([shift={(306:#2)}]u) {#6};
    \node[lnode] (y) at ([shift={(234:#2)}]u) {#7};
    \node[lnode] (z) at ([shift={(162:#2)}]u) {#8};
    \node[lnode,draw=none,fill=none] (dummy) at ([shift={(270:#2)}]u) {};
    \path (u)     edge[bend left=20] (v)
          (v)     edge[bend left=20] (u)
                  edge (w)
          (w.295) edge[bend left=20] (x)
          (x)     edge (u)
          (x.75)  edge[bend left=20] (w.250)
          (y)     edge (u);
  \end{tikzpicture}
}

\newcommand{\squaregraphPic}[6]{
  \begin{tikzpicture}[lgraph,#1]
    \node[lnode] (u) {#3};
    \node[lnode] (v) at ([shift={(315:#2)}]u) {#4};
    \node[lnode] (w) at ([shift={(225:#2)}]v) {#5};
    \node[lnode] (x) at ([shift={(225:#2)}]u) {#6};
    \path (u) edge (v)
              edge (x)
          (w) edge (v)
              edge (x);
  \end{tikzpicture}
}
